Shapley Pruning for Neural Network Compression

Neural network pruning is a rich field with a variety of approaches. In this work, we propose to connect the existing pruning concepts such as leave-one-out pruning and oracle pruning and develop them into a more general Shapley value-based framework that targets the compression of convolutional neural networks. To allow for practical applications in utilizing the Shapley value, this work presents the Shapley value approximations, and performs the comparative analysis in terms of cost-benefit utility for the neural network compression. The proposed ranks are evaluated against a new benchmark, Oracle rank, constructed based on oracle sets. The broad experiments show that the proposed normative ranking and its approximations show practical results, obtaining state-of-the-art network compression.

==> figures/compression_graphs.tex <==
\begin{figure*}[h]
    \centering
 \includegraphics[width=0.3\textwidth]{images/compression_acc_plot_mnist.png}
  \includegraphics[width=0.3\textwidth]{images/compression_acc_plot_fashionmnist.png}
   \includegraphics[width=0.3\textwidth]{images/compression_acc_plot_cifar.png}
    \caption{Comparison to magnitude pruning. The data points are average performance over 1000 architectures binned with respect to the given compression rate.}
    \label{fig:mag_pru}
\end{figure*}

==> tables/table_compression.tex <==
\begin{table}[t]
\small
% \label{tab:table_comp}
    \centering
    \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
    \hline
            {\rowcolor[gray]{0.9}}

        Method & Architecture & Err & Flp & Prm\\
  	\hline
          \textbf{NR} &\textbf{5-7-45-20}&  1.0 & \textbf{130K} & \textbf{4K} \\
          %RDP &4-7-110-66&  1.0\%} \\
        
          BC-GNJ & 8-13-88-13&  1.0 & 284K & 11K\\
          BC-GHS & 5-10-76-16 & 1.0 & 155K & 8K\\
          FDOO & 2-7-112-478&  1.1 &  111K & 242K \\
          (100K) & & & & \\
          FDOO & 3-8-128-499& 1.0 & 153K & 267K\\
        (200K) & & & & \\
           GL & 3-12-192-500&  1.0 & 205K & 288K\\
           GD & 7-13-208-16&  1.1 & 253K & 46K\\
            SBP & 3-18-284-283& \textbf{0.9} & 217K & 163K \\
        \hline
        {\rowcolor[gray]{0.9}}
        Method & Architecture & Err & Flp & Prm\\
        \hline
        \textbf{NR} & \textbf{34-34-68-68-75-106-101-92}  &  &  & \\
        
          & \textbf{-92-102-92-92-67-67-62-62}  & 8.6 & \textbf{44M} & 1.3M}\\
        
        \textbf{NR} & \textbf{39-39-63-48-55-98-97-52}  &  &  & \\ 
        
         & \textbf{-62-22-42-47-47-42-62}  & 9.1 & \textbf{34M} & 0.9M\\ 
        
        %./vgg_retrain_filters[25,25,65,80,201,158,165,467,450,490,470,469,469,476,450].1.out:Test Lossds: 0.552 | Acc: 91.160% (9116/10000)

        
         BC-GNJ & 63-64-128-128-245-155-63-26&  &  &\\
         
            & -24-24-20-14-12-11-15& \textbf{8.3} & 142M & 1.0M\\
        
        
         
          BC-GHS & 51-62-125-128-228-129-38-13 &  &  & \\
          
              & -9-6-5-6-6-20 & 9.0 & 122M & \textbf{0.8M}\\
          \hline
    
    \end{tabular}
    \vspace{0.4cm}
    \caption{The structured pruning of LeNet-5 and VGG-16. Pruned networks are measured in terms of the number of FLoPs (Flp) and the number of parameters (Prm). We benchmark our method (NR) against BC-GNJ, BC-GHS~\cite{louizos2017bayesian}, FDOO(100K,200K)~\cite{tang2018flops}, Generalized Dropout(GD)~\cite{srinivas2015data}, Group Lasso(GL)~\cite{wen2016learning}, 
    Structured Bayesian Pruning(SBP)~\cite{neklyudov2017structured}.
    }
    
    \label{tab:compression_rank}

\vspace{-0.3cm}
\end{table}

==> tables/table_lenet.tex <==


\begin{table}[t]
\captionsetup{font=scriptsize,labelfont=scriptsize}
\scriptsize
%\small
% \label{tab:table_comp}
    \centering
  %  \scriptsize
     \begin{tabular}{ccccc}
    \toprule
            %{\rowcolor[gray]{0.9}}

        Method & Error & FLOPs & Params\\
  	\midrule
          \textbf{Shapley (perm)} & \textbf{1.04} & \textbf{131K} & \textbf{4.5K} \\ 
          
          Dirichlet [\citenum{adamczewski2020dirichlet} & 1.1 & 140K & \ 5.5K \\ 
          
          %RDP &4-7-110-66&  1.0\%} \\
        
          BC-GNJ [\citenum{louizos2017bayesian}] & 1.0 & 288K & 15K\\ 
          BC-GHS [\citenum{louizos2017bayesian}] & 1.0 & 159K & 9K\\ 
          
          RDP [\citenum{oh2019radial}] & 1.0 & 117K & 16K\\  
          FDOO (100K) [\citenum{tang2018flops}] & 1.1 &  \textbf{113K} & 63K \\ 
          %(100K) & & & & \\
          %FDOO (200K) [\citenum{tang2018flops} & 1.0 & 157K & 76K\\ 
        %(200K) & & & & \\
           GL [\citenum{wen2016learning}] &  1.0 & 211K & 112K\\ 
           GD [\citenum{srinivas2015data}] &  1.1 & 273K & 29K\\ 
            SBP [\citenum{neklyudov2017structured}] &  \textbf{0.9 } & 226K & 99K \\ 
            \textbf{Shapley (perm)} & \textbf{0.88} & \textbf{205K} & \textbf{5.9K} \\ 
          Baseline~[\citenum{lecun1998gradient}] & 0.73 & 2549K & 688K \\
        \bottomrule
      
  
%     \begin{tabular}{ccccc}
%     \toprule
%             %{\rowcolor[gray]{0.9}}

%         Method & Architecture & Error & FLOPs & Params\\
%   	\midrule
%           \textbf{Dirichlet (150)} &\textbf{6-8-40-20}&  1.1 & 168K & \textbf{6K} \\ 
          
%           \textbf{Dirichlet (mean)} &\textbf{5-8-45-15}&  1.1 & 140K & \textbf{5.5K} \\ 
          
%           \textbf{Dirichlet (joint)} &\textbf{6-7-35-17}&  1.1 & 158K & \textbf{5.5K} \\ 
%           %RDP &4-7-110-66&  1.0\%} \\
        
%           BC-GNJ & 8-13-88-13&  1.0 & 288K & 15K\\ 
%           BC-GHS & 5-10-76-16 & 1.0 & 159K & 9K\\ 
          
%           RDP & 4-7-110-66 & 1.0 & 117K & 16K\\  
%           FDOO (100K) & 2-7-112-478&  1.1 &  \textbf{113K} & 63K \\ 
%           %(100K) & & & & \\
%           FDOO (200K) & 3-8-128-499& 1.0 & 157K & 76K\\ 
%         %(200K) & & & & \\
%           GL & 3-12-192-500&  1.0 & 211K & 112K\\ 
%           GD & 7-13-208-16&  1.1 & 273K & 29K\\ 
%             SBP & 3-18-284-283& \textbf{0.9} & 226K & 99K \\
%         \bottomrule
      
    
    \end{tabular}
%    \vspace{1cm}

    \caption{ Comparison of pruned models on \textbf{LeNet-5} on MNIST. Top-1 error, computational complexity in terms of FLOPs, and number of parameters are reported.}
    
   %  The pruned network is measured in terms of the number of FLOPs and the number of parameters (Params).
   % The proposed method outperforms the benchmark methods as far as the number of parameters is concerned and it produces the most optimal Params to FLOPs ratio. 
    
    \label{tab:compression_rank}

\end{table}
%\vspace{-0.8cm}
%  We benchmark our method (IS) against RDP~[\citenum{oh2019radial}, BC-GNJ, BC-GHS~[\citenum{louizos2017bayesian}, FDOO (100K,200K)~[\citenum{tang2018flops}, Generalized Dropout (GD)~[\citenum{srinivas2015data}, Group Lasso (GL)~[\citenum{wen2016learning}, 
%     Structured Bayesian Pruning (SBP)~[\citenum{neklyudov2017structured}.




==> tables/table_ranking_comparison.tex <==
\begin{table}[t]

\begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|c|}
\hline
{\rowcolor[gray]{0.9}}
    & L1 & L2 & Der &Rand & \textbf{IS} \\\hline
    \textbf{MNIST}  & 9.2 &9.3 & 8.0 & 13.4 &$\mathbf{7.6}$ \\ \hline
   \textbf{ FashionMNIST} & 11.3 & 11.1 & 11.0 & 12.6 & $\mathbf{9.7}$\\ \hline
   % CIFAR &  & &  & &   \\ \hline
\end{tabular}{}
\caption{The Spearman's foottule distance between the Shapley value ranking and the importance switch ranking (IS) as well as magnitude-based mathods (L1 and L2) and derivative-based method (Der).}

\end{table}

==> tables/table_resnet50_imagenet.tex <==
\begin{table}[!t]
\captionsetup{font=scriptsize,labelfont=scriptsize}
\scriptsize
\centering
%\scriptsize
 %   \begin{center}
 %       \scriptsize
% \vspace{-0.7cm}
        \begin{tabular}{ccc}
            \toprule
            Method  & \shortstack{Error} &  \shortstack{FLOPs Ratio} & %\shortstack{Params Ratio} 
            \\ \midrule
            % \multicolumn{6}{c}{ResNet18, ImageNet} \\ \hline
            % Random &50 &31.36 &11.72 &70.53	&76.1\\
            % \textcolor{red}{FPGM}~[\citenum{he2019filter}	&90	&31.59	&11.52	&58.20	& --	\\
            % \textcolor{red}{SFP}~[\citenum{he2018soft}	&100	&32.90	&12.22	&58.20	& --	\\
            % Random &25 & 34.50 & 13.44 & 50.57 &	68.8 \\

            \textbf{Shapley (regr)} & \textbf{27.4}	& \textbf{59.42}	 %& \textbf{60.42}	
            \\ 
            %SFP~[\citenum{he2018soft}	&25.39	&7.94	&58.2	& --	\\
        GAL-0.5~[\citenum{lin2019towards}]	&28.05		&56.97	
            %& \textbf{83.14}	
            \\
            SSS~[\citenum{huang2018data}]        &28.18     &56.96  
            %&61.15 
            \\
            
          
            
            SFP~[\citenum{he2018soft}]	&25.39		&58.2	
            %& --	
            \\
             %ResRep
            %&24.70 & 62.10 & - \\
            % NISP~[\citenum{yu2018nisp} 	& 90	&	&   &55.99	&	\\
            % Channel Pr 	& 10	&	&9.2	&100	&	\\
            
            %      Random Pruning     &25.85	&8.01   & 50.72 & 54.99	\\
            % Random Pruning   & 75   &25.22	&7.69   & 50.72 & 54.99	\\
            % Random Pruning	 & 120	&24.87	&7.48	& 48.99	& 54.12	\\
         \textbf{Shapley (regr)} & \textbf{25.20}	& \textbf{58.27}	 %& \textbf{60.42}	
            \\ 
            AutoPruner~[\citenum{luo2020autopruner}] 	&25.24	&	48.79	%	&--	
            \\
              HRank~[\citenum{lin2020hrank}] 		&25.02		&56.23	
            %& 63.33	
            \\
            Adapt-DCP~[\citenum{liu2021discrimination}]    &24.85  & 47.59     
            %&45.01
            \\
            {FPGM}~[\citenum{he2019filter}]	            	&25.17	&46.50	%	&--	
            \\
            DCP~[\citenum{zhuang2018discrimination}] 		&25.05	& 44.50	%&48.44	
            \\
            % C-SGD 	&	&25.46	&7.91	&44.24	&	\\
            ThiNet~[\citenum{luo2017thinet}] 		&27.97		&44.17	
            %& --	
            \\ 
            ResRep~[\citenum{ding2021resrep_reb}]
            &\textbf{23.85} & 54.54 
            %& - 
            \\
             Baseline ~[\citenum{paszke2017automatic}] 		&23.87		& 0.00	%&0.00	
             \\ 
            \bottomrule
            % SASL 	& 10	&24.85	&7.53	&43.9	&	\\
            % TRP 	& 10	&27.31	&8.59	&43.48	&	\\
            % LFPC 	&	&25.54	&7.68	&39.2	&	\\
            % ResRep	&	&24.51	&7.45	&37.9	&	\\
            %{MetaPruning}~[\citenum{liu2019metapruning}	 & 24.60	& --	&48.78	& --	\\
            %{AutoSlim}~[\citenum{yu2019autoslim}        & 24.40 & -- & 80.60 & -- \\
            
            
\end{tabular} 
\caption{ Comparison between pruned \textbf{ResNet-50} on Imagenet (right) and the current methods. Top-1 Error and the compression rates are reported. \textbf{Higher ratios} indicate \textbf{higher compression} and smaller models.}
\label{tab:compression_rank_resnet}
 \vspace{-0.4cm}
 \end{table}

==> tables/table_resnet56.tex <==
 \begin{table} [t]
 \captionsetup{font=scriptsize,labelfont=scriptsize}
\scriptsize
\centering
  \begin{tabular}{cccc}
  \toprule
Method & Error & FLOPs & Parameters \\
\midrule
\textbf{Shapley (regr)} & \textbf{8.91}  & \textbf{13.64M}  & \textbf{0.24M }\\
Dirichlet [\citenum{adamczewski2020dirichlet}] & 9.13 & 13.64M & 0.24M \\
Hinge~[\citenum{li2020group}] & 7.35 & 30.58M & 0.18M \\
Hrank [\citenum{lin2020hrank}] & 9.28 & 32.53M & 0.27M\\
\textbf{Shapley (kern)} & \textbf{6.82}  & \textbf{46.38M}  & \textbf{0.34M} \\
DHP~[\citenum{li2020dhp}] & 7.06 & 49.78M & 0.35M \\
GAL-0.8 [\citenum{lin2019towards}] & 9.64 & 49.99M & 0.29M \\
KSE [\citenum{li2019exploiting}] & 7.12 & 50M & 0.36M \\
CP [\citenum{he2017channel}] & 9.20 & 62M & - \\
NISP~[\citenum{yu2018nisp}] & 6.99 & 81M & 0.49M \\
Baseline~[\citenum{he2016deep}] & 7.05 &127.4M &0.86M \\
\bottomrule
\end{tabular} 
%\vspace{0.2cm}

\caption{Comparison between pruned \textbf{ResNet-56} on CIFAR-10 (left) and the benchmarks. Top-1 Error and the compressed model parameters and FLOPs are reported.}
\label{tab:compression_rank_resnet}
% \vspace{-0.5cm}
\end{table}

==> tables/table_resnet56resnet50.tex <==
 \begin{table*} [h]
 %\captionsetup{font=scriptsize,labelfont=scriptsize}

 \parbox{.45\linewidth}{
\centering
  \begin{tabular}{cccc}
  \toprule
Method & Error & FLOPs & Parameters \\
\midrule
\textbf{Shapley (regr)} & \textbf{8.91}  & \textbf{13.64M}  & \textbf{0.24M }\\
Dirichlet [\citenum{adamczewski2020dirichlet}] & 9.13 & 13.64M & 0.24M \\
Hinge~[\citenum{li2020group}] & 7.35 & 30.58M & 0.18M \\
Hrank [\citenum{lin2020hrank}] & 9.28 & 32.53M & 0.27M\\
\textbf{Shapley (kern)} & \textbf{6.82}  & \textbf{46.38M}  & \textbf{0.34M} \\
DHP~[\citenum{li2020dhp}] & 7.06 & 49.78M & 0.35M \\
GAL-0.8 [\citenum{lin2019towards}] & 9.64 & 49.99M & 0.29M \\
KSE [\citenum{li2019exploiting}] & 7.12 & 50M & 0.36M \\
CP [\citenum{he2017channel}] & 9.20 & 62M & - \\
NISP~[\citenum{yu2018nisp}] & 6.99 & 81M & 0.49M \\
RRCP~[\citenum{li2022revisiting}] & 6.52 & 62.38M & 0.35M \\
Baseline~[\citenum{he2016deep}] & 7.05 &127.4M &0.86M \\
\bottomrule
\end{tabular} 
\vspace{0.2cm}

\caption{Comparison between pruned \textbf{ResNet-56} on CIFAR-10 (left) and the benchmarks. Top-1 Error and the compressed model parameters and FLOPs are reported.}
\label{tab:compression_rank_resnet56}
% \vspace{-0.5cm}
} %parbox
\hfill
%\captionsetup{font=scriptsize,labelfont=scriptsize}
\parbox{.45\linewidth}{
\centering
        \begin{tabular}{ccc}
            \toprule
            Method  & \shortstack{Error} &  \shortstack{FLOPs Ratio} & %\shortstack{Params Ratio} 
            \\ \midrule
            % \multicolumn{6}{c}{ResNet18, ImageNet} \\ \hline
            % Random &50 &31.36 &11.72 &70.53	&76.1\\
            % \textcolor{red}{FPGM}~[\citenum{he2019filter}	&90	&31.59	&11.52	&58.20	& --	\\
            % \textcolor{red}{SFP}~[\citenum{he2018soft}	&100	&32.90	&12.22	&58.20	& --	\\
            % Random &25 & 34.50 & 13.44 & 50.57 &	68.8 \\

            \textbf{Shapley (regr)} & \textbf{27.4}	& \textbf{59.42}	 %& \textbf{60.42}	
            \\ 
            %SFP~[\citenum{he2018soft}	&25.39	&7.94	&58.2	& --	\\
        GAL-0.5~[\citenum{lin2019towards}]	&28.05		&56.97	
            %& \textbf{83.14}	
            \\
            SSS~[\citenum{huang2018data}]        &28.18     &56.96  
            %&61.15 
            \\
            
          
            
            SFP~[\citenum{he2018soft}]	&25.39		&58.2	
            %& --	
            \\
             %ResRep
            %&24.70 & 62.10 & - \\
            % NISP~[\citenum{yu2018nisp} 	& 90	&	&   &55.99	&	\\
            % Channel Pr 	& 10	&	&9.2	&100	&	\\
            
            %      Random Pruning     &25.85	&8.01   & 50.72 & 54.99	\\
            % Random Pruning   & 75   &25.22	&7.69   & 50.72 & 54.99	\\
            % Random Pruning	 & 120	&24.87	&7.48	& 48.99	& 54.12	\\
         \textbf{Shapley (regr)} & \textbf{25.20}	& \textbf{58.27}	 %& \textbf{60.42}	
            \\ 
             RRCP~[\citenum{li2022revisiting}] 	&25.22	&	48.79	%	&--	
            \\
            AutoPruner~[\citenum{luo2020autopruner}] 	&25.24	&	48.79	%	&--	
            \\
              HRank~[\citenum{lin2020hrank}] 		&25.02		&56.23	
            %& 63.33	
            \\
            Adapt-DCP~[\citenum{liu2021discrimination}]    &24.85  & 47.59     
            %&45.01
            \\
            {FPGM}~[\citenum{he2019filter}]	            	&25.17	&46.50	%	&--	
            \\
            DCP~[\citenum{zhuang2018discrimination}] 		&25.05	& 44.50	%&48.44	
            \\
            % C-SGD 	&	&25.46	&7.91	&44.24	&	\\
            ThiNet~[\citenum{luo2017thinet}] 		&27.97		&44.17	
            %& --	
            \\ 
                ANP~[\citenum{lin2020improved}] 	&23.93	&	48.79	%	&--	
            \\
            ResRep~[\citenum{ding2021resrep_reb}]
            &\textbf{23.85} & 54.54 
            %& - 
            \\
             Baseline ~[\citenum{paszke2017automatic}] 		&23.87		& 0.00	%&0.00	
             \\ 
            \bottomrule
            % SASL 	& 10	&24.85	&7.53	&43.9	&	\\
            % TRP 	& 10	&27.31	&8.59	&43.48	&	\\
            % LFPC 	&	&25.54	&7.68	&39.2	&	\\
            % ResRep	&	&24.51	&7.45	&37.9	&	\\
            %{MetaPruning}~[\citenum{liu2019metapruning}	 & 24.60	& --	&48.78	& --	\\
            %{AutoSlim}~[\citenum{yu2019autoslim}        & 24.40 & -- & 80.60 & -- \\
            
        
\end{tabular} 
 \vspace{0.2cm}

\caption{ Comparison between pruned \textbf{ResNet-50} on Imagenet (right) and the current methods. Top-1 Error and the compression rates are reported. \textbf{Higher ratios} indicate \textbf{higher compression} and smaller models.}

} %parbox
 \label{tab:compression_rank_resnet50a}   
 \vspace{0.4cm}
 \end{table*}

==> tables/table_test.tex <==
\begin{table}[!tbp]
  \centering
  \begin{subtable}[t]{0.4\textwidth}
    \begin{center}
      \begin{tabular}{ccc}
        \hline
        a&b&c\\
        \hline
      \end{tabular}
      \caption{Table at left.}
      \label{tab:left}
    \end{center}
  \end{subtable}
  \quad
  \begin{subtable}[t]{0.4\textwidth}
    \begin{center}
      \begin{tabular}{ccc}
        \hline
        d&e&f\\
        \hline
      \end{tabular}
      \caption{Table at right.}
      \label{tab:right}
    \end{center}
  \end{subtable}
  \caption{This contains two subtables.}
  \label{tab:main}
\end{table}

==> tables/table_vgg.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{figure}[ht!]
%\vspace{-3mm}

 % \begin{subfigure}{0.5\textwidth}

\begin{table}[t]
\captionsetup{font=scriptsize,labelfont=scriptsize}
\scriptsize
  \centering
 % \scriptsize
  \begin{tabular}{cccc}
  \toprule
Method & Error & FLOPs & Parameters \\
\midrule
\textbf{Shapley (perm)} & \textbf{7.91} & \textbf{43.0M} & \textbf{0.68M} \\
Dirichlet [\citenum{adamczewski2020dirichlet}] & 8.48 & \textbf{38.0M} & 0.84M \\
Hrank [\citenum{lin2020hrank}] & 8.77 & 73.7M  & 1.78M  \\
BC-GNJ [\citenum{louizos2017bayesian}] & 8.3 & 142M &  1.0M \\
BC-GHS [\citenum{louizos2017bayesian}] & 9.0 & 122M & 0.8M  \\
RDP [\citenum{oh2019radial}] & 8.7 & 172M & 3.1M  \\
GAL-0.05 [\citenum{lin2019towards}] & 7.97 & 189.5M  & 3.36M  \\
SSS [\citenum{huang2018data}] & 6.98 & 183.1M  & 3.93M  \\
VP [\citenum{zhao2019variational}] & 5.72 & 190M & 3.92M  \\
\textbf{Shapley (perm)} & \textbf{5.67} & \textbf{109.0M} & \textbf{3.7M} \\
Baseline~[\citenum{simonyan2014very}] & 5.36 & 313.7M & 15M \\
\bottomrule
\end{tabular}
%\vspace{1cm}
\caption{ Comparison of pruned models on \textbf{VGG-16} on CIFAR-10. Notice that the more accurate models are also considerably larger.}
\label{tab:compression_rank_vgg}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% \begin{table*}[ht!]
% %\small
% % \label{tab:table_comp}
%     \centering
%   % \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
%      \begin{tabular}{ccccc}
%     \midrule
%         %{\rowcolor[gray]{0.9}}
%         Method & Architecture & Error & FLOPs & Params\\
%         \hline
%          \textbf{Dirichlet (50)} & \textbf{39-39-63-48-55-88-87-52-62-22-42-47-47-47}   & 8.6 & \bf{46M} & \bf{0.7M}\\
        
        
%         %\hdashline
        
%         \textbf{Dirichlet (mean)} & \textbf{34-34-68-68-75-106-101-92-102-92-92-67-67-62-62}  & 8.6 & \bf{46M} & \bf{0.7M}\\
        
%         %\hdashline
%         % \textbf{IS} & \textbf{39-39-63-48-55-98-97-52}  &  &  & \\ 
        
%         %  & \textbf{-62-22-42-47-47-42-62}  & 9.1 & \textbf{34M} & 0.9M\\  \hdashline
        
%         %[39, 39, 63, 48, 55, 88, 87, 52, 62, 22, 42, 47, 47, 47, 10]
        
%         %./vgg_retrain_filters[25,25,65,80,201,158,165,467,450,490,470,469,469,476,450].1.out:Test Lossds: 0.552 | Acc: 91.160% (9116/10000)
        
%         %\hdashline
        
%          BC-GNJ & 63-64-128-128-245-155-63-26  -24-24-20-14-12-11-15&  8.3 & 142M & 1.0M\\
         
        
        
        
%          %\hdashline
%           BC-GHS & 51-62-125-128-228-129-38-13-9-6-5-6-6-20 & 9.0 & 122M & 0.8M\\
          
             
%         %\hdashline
        
%         RDP  & 27-57-125-122-236-244-246-340-127-77-89-52-380-414&  8.7  & 172M & 3.1M \\ 
              
%           \bottomrule
    
%     \end{tabular}
%     %\vspace{0.5cm}
%     \caption{The structured pruning of  \textbf{VGG-16}. Our method using $50$ posterior samples for switches achieved the best compression performance in terms of both FLOPs and the number of parameters with a significantly lower error rate, compared to other existing methods.
%     }
    
%     \label{tab:compression_rank_vgg}

% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[h!]
% %\small
% % \label{tab:table_comp}
%     \centering
%   % \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
%      \begin{tabular}{ccccc}
%     \midrule
%         %{\rowcolor[gray]{0.9}}
%         Method & Architecture & Error & Comp. Rate & Params\\
%         \hline
        
%          \textbf{Dirichlet } & \textbf{65,75,70,90,149,149,164,149,305,325,304,306}   & 
%          4.5 & 52.2\% 
%          & \textbf{17.4M}\\
        
%         $L_0$ ARM [\citenum{li2019l_0} & \text{82-75-82-87-164-169-156-161-317-317-317-324}  & 
%         4.4 & $49.9\%$
%         & 18.3M\\
        
%         $L_0$ ARM [\citenum{li2019l_0} & 75-72-78-78-157-165-131-162-336-325-331-343 & \textbf{4.3} & $49.6\%$ & 18.4M\\
        
         
              
%           \bottomrule
    
%     \end{tabular}
%     %\vspace{0.5cm}
%     \caption{The structured pruning of \textbf{WideResNet-28-10}. Compared to $L_0$-ARM, with a slight increase in the error rate, our method achieves the smallest number of parameters. 
%     }
    
%     \label{tab:compression_rank_wrn}

% \end{table*}






%%%%%%%%%%%%%%%%
%TWO LINE

% \begin{table}[t]
% %\small
% % \label{tab:table_comp}
%     \centering
%   % \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
%      \begin{tabular}{ccccc}
%     \midrule
%         %{\rowcolor[gray]{0.9}}
%         Method & Architecture & Error & FLOPs & Params\\
%         \hline
%          \textbf{IS (50)} & \textbf{39-39-63-48-55-88-87-52}  &  &  & \\
        
%           & \textbf{-62-22-42-47-47-47}  & \textbf{7.9} & \textbf{38M} & \textbf{0.3M}}\\
          
        
%         \hdashline
        
%         \textbf{IS (mean)} & \textbf{34-34-68-68-75-106-101-}  &  &  & \\
        
%           & \textbf{-92-102-92-92-67-67-62-62}  & 8.6 & 46M & 0.7M}\\
        
%         \hdashline
%         % \textbf{IS} & \textbf{39-39-63-48-55-98-97-52}  &  &  & \\ 
        
%         %  & \textbf{-62-22-42-47-47-42-62}  & 9.1 & \textbf{34M} & 0.9M\\  \hdashline
        
%         %[39, 39, 63, 48, 55, 88, 87, 52, 62, 22, 42, 47, 47, 47, 10]
        
%         %./vgg_retrain_filters[25,25,65,80,201,158,165,467,450,490,470,469,469,476,450].1.out:Test Lossds: 0.552 | Acc: 91.160% (9116/10000)
        
%         \hdashline
        
%          BC-GNJ & 63-64-128-128-245-155-63-26&  &  &\\
         
%             & -24-24-20-14-12-11-15& 8.3 & 142M & 1.0M\\
        
        
%          \hdashline
%           BC-GHS & 51-62-125-128-228-129-38-13 &  &  & \\
          
%               & -9-6-5-6-6-20 & 9.0 & 122M & 0.8M\\
%         \hdashline
        
%         RDP  & 27-57-125-122-236-244-246& &  &  \\
%          & -340-127-77-89-52-380-414&  8.7  & 172M & 3.1M \\      
%           \bottomrule
    
%     \end{tabular}
%     %\vspace{0.5cm}
%     \caption{The structured pruning of  VGG-16. Our method using $50$ posterior samples for switches achieved the best compression performance in terms of both FLOPs and the number of parameters with a significantly lower error rate, compared to other existing methods.
%     }
    
%     \label{tab:compression_rank_vgg}

% \end{table}
